Extra Global Attention Designation Using Keyword Detection in Sparse Transformer Architectures

In this paper, we propose an extension to Longformer Encoder-Decoder, a popular sparse transformer architecture. One common challenge with sparse transformers is that they can struggle with encoding of long range context, such as connections between topics discussed at a beginning and end of a document. A method to selectively increase global attention is proposed and demonstrated for abstractive summarization tasks on several benchmark data sets. By prefixing the transcript with additional keywords and encoding global attention on these keywords, improvement in zero-shot, few-shot, and fine-tuned cases is demonstrated for some benchmark data sets.

==> oldTables.tex <==

\begin{table}
\centering
\caption{Zero shot results with AMI data set\label{AMIzeroShot}}
%%% \tablesize{} %% You can specify the fontsize here, e.g., \tablesize{\footnotesize}. If commented out \small will be used.
\begin{tabular}{|p{3.5cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|}
\toprule
\textbf{Keyword Count}	& \textbf{ROUGE-1}	& \textbf{ROUGE-2} & \textbf{ROUGE-L}\\
\midrule
Baseline		& 19.2	& 3.2 & 9.8\\
\midrule
5 keywords		& 20.8		& 3.6 & 10.2\\
\midrule
10 keywords		& 21.1	& 3.5 & 10.2\\
\midrule
20 keywords		& 21.5	& 4.1 & 10.4\\
\midrule
50 keywords		& 22.4	& 3.8 & 10.9\\
\midrule
5 random keywords		& 20.3		& 3.1 & 9.8\\
\midrule
10 random keywords		& 21.9	& 3.3 & 10.7\\
\midrule
20 random keywords		& 20.7	& 3.9 & 9.9\\
\midrule
50 random keywords		& 20.4	& 3.4 & 9.8\\
\bottomrule
\end{tabular}
\end{table}





\begin{table}
\centering
\caption{Zero shot results with ICSI data set\label{ICSIzeroShot}}
%%% \tablesize{} %% You can specify the fontsize here, e.g., \tablesize{\footnotesize}. If commented out \small will be used.
\begin{tabular}{p{3.5cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}}
\hline\hline
\textbf{Keyword Count}	& \textbf{ROUGE-1}	& \textbf{ROUGE-2} & \textbf{ROUGE-L}\\
\hline
Baseline		& 18.0	& 1.8 & 8.7\\
%\hline
5 keywords		& 15.4		& 1.3 & 7.8\\
%\hline
10 keywords		& 15.2	& 1.5 & 6.3\\
%\hline
20 keywords		& 9.8	& 1.1 & 4.2\\
%\hline
50 keywords		& 15.8	& 2.0 & 6.9\\
%\hline
5 random keywords		& 10.7		& 0.9 & 5.3\\
%\hline
10 random keywords		& 8.0	& 0.9 & 5.3\\
%\hline
20 random keywords		& 14.9	& 1.5 & 7.0\\
%\hline
50 random keywords		& 9.8	& 1.4 & 4.8\\
\hline
\end{tabular}
\end{table}






\begin{table}
\centering
\caption{Zero shot results with arXiv data set\label{arXivzeroShot}}
%%% \tablesize{} %% You can specify the fontsize here, e.g., \tablesize{\footnotesize}. If commented out \small will be used.
\begin{tabular}{|p{3.5cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|}
\toprule
\textbf{Keyword Count}	& \textbf{ROUGE-1}	& \textbf{ROUGE-2} & \textbf{ROUGE-L}\\
\midrule
Baseline (base)		& 14.4	& 3.4 & 9.4\\
\midrule
10 keywords (base)		& 10.0	& 2.2 & 6.6\\
\midrule
20 keywords (base)		& 8.1	& 2.0 & 5.5\\
\midrule
Baseline (arXiv pretrain)	& 43.3	& 19.0 & 25.6\\
\midrule
10 keywords (arXiv pretrain)		& 44.1	& 19.4 & 26.3\\
\midrule
20 keywords (arXiv pretrain)		& 43.8	& 18.7 & 25.7\\
\bottomrule
\end{tabular}
\end{table}







\begin{table}
\centering
\caption{Fine tuned results with AMI data set\label{AMIfineTune}}
%%% \tablesize{} %% You can specify the fontsize here, e.g., \tablesize{\footnotesize}. If commented out \small will be used.
\begin{tabular}{|p{3.5cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|}
\toprule
\textbf{Keyword Count}	& \textbf{ROUGE-1}	& \textbf{ROUGE-2} & \textbf{ROUGE-L}\\
\midrule
Baseline		& 46.1	& 17.4 & 23.1\\
\midrule
5 keywords		& 46.5	& 17.6 & 23.3\\
\midrule
10 keywords		& 46.6	& 16.9 & 23.1\\

\midrule
20 keywords		& 46.7	& 17.0 & 24.1\\
\midrule
50 keywords		& 48.5	& 17.7 & 23.7\\
\midrule
100 keywords		& 48.4	& 17.4 & 23.3\\
\midrule
10 random keywords		& 41.8	& 15.6 & 23.3\\
\bottomrule
\end{tabular}
\end{table}








\begin{table}
\centering
\caption{Fine tuned results with ICSI data set\label{ICSIfineTune}}
%%% \tablesize{} %% You can specify the fontsize here, e.g., \tablesize{\footnotesize}. If commented out \small will be used.
\begin{tabular}{|p{3.5cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|}
\toprule
\textbf{Keyword Count}	& \textbf{ROUGE-1}	& \textbf{ROUGE-2} & \textbf{ROUGE-L}\\
\midrule
Baseline		& 45.5	& 13.3 & 19.2\\

\midrule
10 keywords		& 40.0	& 11.8 & 18.1\\

\midrule
20 keywords		& 40.9	& 11.8 & 18.0\\
\midrule
50 keywords		& 38.9	& 12.0 & 17.7\\
\midrule
100 keywords		& 38.8	& 11.9 & 17.0\\
\midrule
20 random keywords		& 40.8	& 12.4 & 18.1\\
\bottomrule
\end{tabular}
\end{table}





\begin{table}
\centering
\caption{Fine tuned results with arXiv data set\label{arXivfineTune}}
%%% \tablesize{} %% You can specify the fontsize here, e.g., \tablesize{\footnotesize}. If commented out \small will be used.
\begin{tabular}{|p{3.5cm}|p{1.9cm}|p{1.9cm}|p{1.9cm}|}
\toprule
\textbf{Keyword Count}	& \textbf{ROUGE-1}	& \textbf{ROUGE-2} & \textbf{ROUGE-L}\\
\midrule
Baseline (base)		& 37.5	& 11.9 & 20.0\\
\midrule
10 keywords (base)		& 37.4	& 13.8 & 20.0\\
\midrule
20 keywords (base)		& xx.x	& xx.x & xx.x\\

\midrule
Baseline (arXiv fine-tuned)		& 41.3	& 15.5 & 22.1\\


\midrule
10 keywords (arXiv fine-tuned)		& 37.8	& 13.7 & 19.9\\
\midrule
20 keywords	(arXiv fine-tuned)	& 39.6	& 14.7 & 21.2\\

\bottomrule
\end{tabular}
\end{table}



